Large-scale Urban Facility Location Selection with Knowledge-informed Reinforcement Learning

The facility location problem (FLP) is a classical combinatorial optimization challenge aimed at strategically laying out facilities to maximize their accessibility. In this paper, we propose a reinforcement learning method tailored to solve large-scale urban FLP, capable of producing near-optimal solutions at superfast inference speed. We distill the essential swap operation from local search, and simulate it by intelligently selecting edges on a graph of urban regions, guided by a knowledge-informed graph neural network, thus sidestepping the need for heavy computation of local search. Extensive experiments on four US cities with different geospatial conditions demonstrate that our approach can achieve comparable performance to commercial solvers with less than 5\% accessibility loss, while displaying up to 1000 times speedup. We deploy our model as an online geospatial application at https://huggingface.co/spaces/randommmm/MFLP.

==> related.tex <==
% \vspace{-10px}
\section{Related Work}
\noindent\textbf{Machine Learning for Combinatorial Optimization (ML4CO).}
The rise of data mining since the early 2010s has led to the emergence of ML4CO~\cite{zhang2023survey,vinyals2015pointer,li2018combinatorial,khalil2017learning,prates2019learning,zong2022rbg,fan2020finding,kool2018attention,zheng2021combining,hudson2021graph,lin2021pareto,bi2022learning,qiu2022dimes,meirom2021controlling,duan2020efficiently,li2023hardsatgen,chen2019data,geng2023gal} which harnesses ML techniques to tackle complex CO problems in a data-driven paradigm. 
Supervised learning were initially adopted to resolve CO challenges, such as the seminal work of Pointer Network~\cite{vinyals2015pointer} which employed sequence-to-sequence learning to address the Travelling Salesman Problem (TSP).
Particularly, since graphs offer an unified discrete data form to describe CO problems, a series of ML4CO approaches based on GNN~\cite{kipf2016semi,khalil2017learning,li2018combinatorial,hudson2021graph,prates2019learning} were proposed, which are recently combined with self-supervised learning~\cite{wang2022towards} and diffusion models~\cite{sun2023difusco}.
% learning representations of the problem to support policy-making, 
Meanwhile, many CO problems can be formulated as an MDP thereby amenable to resolution through RL~\cite{mnih2015human,schulman2017proximal,meirom2021controlling,fan2020finding,zong2022rbg,kurin2020can,jiang2023ensemble,pan2023adjustable,geng2023gal}.
For example, Meirom \textit{et al}~\cite{meirom2021controlling} proposed a GNN based RL method that controls dynamics on the graph to addresses the influence maximization (IM) problem.
ML4CO methods replace tedious computation such as exact local search with fast inference of neural networks, which are much faster than traditional heuristics or commercial solvers and displays superior scalability to large practical CO problems.
However, many CO problems encapsulate rich domain knowledge, while current ML4CO approaches rarely incorporate the prior knowledge, leading to serious performance degradation that questions their deployment in real applications.
Different from existing approaches, in this paper we develop an ML4CO method that takes the valuable prior knowledge of the specific MFLP into consideration, and deploy the algorithm as an online service that achieves a better trade-off between performance and efficiency.




\noindent\textbf{Facility Location Problem (FLP).}
FLP is a classical CO problem recognized as NP-hard~\cite{shmoys1997approximation,farahani2009facility,owen1998strategic,celik2020comparative}, where $p$ facilities are strategically placed among $N$ candidates to minimize the demand-weighted distance between demand nodes and their nearest facilities~\cite{reese2006solution,maranzana1964location}.
% Solving FLP has a widespread impact in real-world geospatial applications, particularly in urban scenarios where optimized distances directly reflect the accessibility to essential urban services.
Traditionally, FLP is addressed using heuristics and meta-heuristics based on exact local search~\cite{charikar2005improved,arya2001local,kariv1979algorithmic,gwalani2021evaluation,jain2002new,korupolu2000analysis,resende2007fast}.
Heuristics like tabu search~\cite{rolland1997efficient} and variable neighbor search (VNS)~\cite{hansen1997variable} were proposed to promote exploration and avoid trapping at a local optimum.
% Resende \textit{et al}~\cite{resende2007fast} proposed POPSTAR that integrates multi-start solutions with path relinking to discover potential optimal solutions.
Meanwhile, FLP can be framed as MIP thus addressable via commercial solvers like Gurobi~\cite{gurobi} and MOSEK~\cite{andersen2000mosek}.
However, both heuristics and solvers are excessively time-consuming for practical scenarios owing to heavy computation, thus failing to scale up to real-world urban FLP applications.
To accelerate solution generation, ML4CO approaches were developed for solving FLP~\cite{wang2022towards,wang2023solving,matis2023reinforcement,luo2023facility,guo2023swap}, which sidesteps costly local search by approximating with neural networks.
For example, Wang \textit{et al}~\cite{wang2022towards} proposed CardNN, an end-to-end neural solver encoding constraints into neural networks in a self-supervised manner.
% , which can effectively generate FLP solutions in one-shot.
Nevertheless, current ML4CO methods exhibit serious degradation in solution quality and insufficient speedup for deployment in real-world applications.
In contrast, our proposed knowledge-informed neural solver displays comparable accessibility performance to commercial solvers with up to 1000 times speedup, thereby effectively support practical deployment.










